The Type I Superluminous Supernova Catalog I: Light Curve Properties, Models, and Catalog Description

We present the most comprehensive catalog to date of Type I Superluminous Supernovae (SLSNe), a class of stripped envelope supernovae (SNe) characterized by exceptionally high luminosities. We have compiled a sample of 262 SLSNe reported through 2022 December 31. We verified the spectroscopic classification of each SLSN and collated an exhaustive data set of UV, optical and IR photometry from both publicly available data and our own FLEET observational follow-up program, totaling over 30,000 photometric detections. Using these data we derive observational parameters such as the peak absolute magnitudes, rise and decline timescales, as well as bolometric luminosities, temperature and photospheric radius evolution for all SLSNe. Additionally, we model all light curves using a hybrid model that includes contributions from both a magnetar central engine and the radioactive decay of $^{56}$Ni. We explore correlations among various physical and observational parameters, and recover the previously found relation between ejecta mass and magnetar spin, as well as the overall progenitor pre-explosion mass distribution with a peak at $\approx 6.5$ M$_\odot$. We find no significant redshift dependence for any parameter, and no evidence for distinct sub-types of SLSNe. We find that $< 3$\% of SLSNe are best fit with a significant contribution from radioactive decay $\gtrsim 50$\%, representing a set of relatively dim and slowly declining SNe. We provide several analytical tools designed to simulate typical SLSN light curves across a broad range of wavelengths and phases, enabling accurate K-corrections, bolometric scaling calculations, and inclusion of SLSNe in survey simulations or future comparison works. The complete catalog, including all of the photometry, models, and derived parameters, is made available as an open-source resource on GitHub.

==> mycommands.tex <==
% New Commands
\newcommand{\tc}[2][red]{\textcolor{#1}{\emph{\textbf{#2}}}}
\newcommand{\ksmag}{\emph{Ks}~magnitudes }
\newcommand{\jmag}{\emph{J}~magnitudes }
\newcommand{\kpmags}{\emph{Kp}~magnitudes }
\newcommand{\kpmag}{\emph{Kp}~magnitude }
\newcommand{\teff}{\ensuremath{T_{\mathrm{eff}}}}
\newcommand{\logg}{\ensuremath{\log g}}
\newcommand{\kepler}{{\em Kepler}\xspace}
\def\msun{{\rm\,M_\odot}}
\def\rsun{{\rm\,R_\odot}}
\def\mearth{{\rm\,M_\oplus}}
\def\rearth{{\rm\,R_\oplus}}
\def\fearth{{\rm\,F_\oplus}}
\def\lsun{{\rm\,L_\odot}}
\newcommand{\hho}{H$_2$O}
\newcommand{\hh}{H$_2$}
\newcommand{\oo}{O$_2$}
\newcommand{\chhhh}{CH$_4$}
\newcommand{\mjup}{{\rm M}_{\rm Jup}}
\newcommand{\kms}{\rm km\ s^{-1}}
\newcommand{\mps}{\rm m\ s^{-1}}
\newcommand{\cspg}{\rm\ cm^2\ g^{-1}}
\newcommand{\ergs}{\rm\ erg\ s^{-1}}
\newcommand{\kelvin}{\rm K}
\newcommand{\angstrom}{\rm \AA}
\newcommand{\oneday}{\rm day}
\newcommand{\days}{\rm days}
\newcommand{\hours}{\rm hours}
\newcommand{\meter}{\rm m}
\newcommand{\HST}{{\it HST}}
\newcommand{\hubble}{{\it HST}}
\newcommand{\spitzer}{{\it Spitzer}}
\newcommand{\fermi}{{\it Fermi}}
\newcommand{\swift}{{\it Swift}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\mosfit}{{\tt MOSFiT}}
\newcommand{\zeroth}{$0^{\rm th}$}
\newcommand{\first}{$1^{st}$}
\newcommand{\second}{$2^{nd}$}
\newcommand{\third}{$3^{rd}$}
\newcommand{\fourth}{$4^{th}$}
\newcommand{\e}{${\rm e^{-}}$}
\newcommand{\persecond}{${\rm s^{-1}}$}
\newcommand{\perpixel}{${\rm pixel^{-1}}$}
\newcommand{\divideoot}{{\tt divide-oot}}
\newcommand{\modelramp}{{\tt model-ramp}}
\newcommand{\chisq}{$\chi^2$}
\newcommand{\calwf}{{\tt calwf3}}
\newcommand{\rp}{$R_{p}$}
\newcommand{\rs}{$R_{\star}$}
\newcommand{\flt}{{\tt flt}}
\definecolor{orange}{rgb}{.8,0.4,0}
\newcommand{\question}[1]{\sffamily {\em {\color{orange} [#1]}}\normalfont}
\newcommand{\todo}[1]{\sffamily {\em {\color{orange} #1}}\normalfont}
\newcommand{\mad}{\rm MAD}
\newcommand{\Mej}{M_{\rm ej}}
\newcommand{\vej}{v_{\rm ej}}
\newcommand{\apx}{\ensuremath{\sim}}
\newcommand{\WFDD}{{\tt WFDD}}
\newcommand{\WFDM}{{\tt WFDM}}
\newcommand{\WFDR}{{\tt WFDR}}

% Alternate Itemize
\newcommand{\outline}[1]{
\todo{\begin{itemize}
#1
\end{itemize}}}

% AutoRef Stuff
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section}

\renewcommand*{\sectionautorefname}{Section} 
\renewcommand*{\subsectionautorefname}{Section} 

% Citation Alias
\defcitealias{LP98}{LP98}
\defcitealias{CowpBerger15}{CB15}

